MPIrigen: MPI Code Generation through Domain-Specific Language Models

The imperative need to scale computation across numerous nodes highlights the significance of efficient parallel computing, particularly in the realm of Message Passing Interface (MPI) integration. The challenging parallel programming task of generating MPI-based parallel programs has remained unexplored. This study first investigates the performance of state-of-the-art language models in generating MPI-based parallel programs. Findings reveal that widely used models such as GPT-3.5 and PolyCoder (specialized multi-lingual code models) exhibit notable performance degradation, when generating MPI-based programs compared to general-purpose programs. In contrast, domain-specific models such as MonoCoder, which are pretrained on MPI-related programming languages of C and C++, outperform larger models. Subsequently, we introduce a dedicated downstream task of MPI-based program generation by fine-tuning MonoCoder on HPCorpusMPI. We call the resulting model as MPIrigen. We propose an innovative preprocessing for completion only after observing the whole code, thus enabling better completion with a wider context. Comparative analysis against GPT-3.5 zero-shot performance, using a novel HPC-oriented evaluation method, demonstrates that MPIrigen excels in generating accurate MPI functions up to 0.8 accuracy in location and function predictions, and with more than 0.9 accuracy for argument predictions. The success of this tailored solution underscores the importance of domain-specific fine-tuning in optimizing language models for parallel computing code generation, paving the way for a new generation of automatic parallelization tools. The sources of this work are available at our GitHub MPIrigen repository: https://github.com/Scientific-Computing-Lab-NRCN/MPI-rigen

==> plots/mpir.tex <==
\begin{figure*}
  \centering
  
  \begin{subfigure}{\textwidth}
    \centering
    \includegraphics[width=1\linewidth, height=6.2cm]{plots/comp700M_scores_var_0-2.png}
    \caption{\mpir{} (fine-tuned \mono{}-0.7B over 16K MPI codes from \mpicorpus{})}
    \label{fig:subfig1}
  \end{subfigure}

  % \begin{subfigure}{\textwidth}
  %   \centering
  %   \includegraphics[width=1\linewidth]{plots/comp2.7B_scores_var_0-2.png}
  %   \caption{\mono{}-2.7B}
  %   \label{fig:subfig2}
  % \end{subfigure}

  \begin{subfigure}{\textwidth}
    \centering
    \includegraphics[width=1\linewidth, height=6.2cm]{plots/GPT3.5_scores_var_0-2.png}
    \caption{GPT3.5 prompt engineering "Generate the optimal MPI functions for the provided code, and supply in the response the entire complete code with those MPI functions: [CODE]".}
    \label{fig:subfig3}
  \end{subfigure}

  \caption{Comparative analysis of \mpir{} (fine-tuned \mono{}-0.7B over \mpicorpus{} for the MPI calls predictions) and GPT3.5 prompt engineering, demonstrates that \mpir{} excels in generating accurate MPI codes in a breakdown to locations, functions, and arguments. Functions accuracy is measured for matched locations only and arguments accuracy for matched functions only. The results are given as a function of the amount of original MPI calls (1-20), showcasing that accuracy drops as complexity grows (besides the ultra simplicity of one or two MPI function calls).}
  \label{fig:mpir}
\end{figure*}


==> plots/pi_tokompiler_comparison.tex <==
% \begin{figure*}[h]
%     \centering
%     \begin{subfigure}[b]{0.44\textwidth}
% \begin{lstlisting}[breaklines=true, breakatwhitespace=true, basicstyle=\footnotesize\ttfamily, columns=fullflexible]
% int main(argc,argv)
% {
%     int done = 0, n = 10000, rank, numprocs, i;
%     double pi_total, pi, h, sum, x;

%     MPI_Init(&argc,&argv);
%     MPI_Comm_size(MPI_COMM_WORLD,&numprocs);
%     MPI_Comm_rank(MPI_COMM_WORLD,&rank);

%     while (!done)
%     {
% 	   MPI_Bcast(&n, 1, MPI_INT, 0, MPI_COMM_WORLD);
% 	   if (n == 0) 
%               break;
% 	   h   = 1.0 / (double) n;...
% \end{lstlisting}        
% \caption{Source code}
%         \label{fig:subifg1}
%     \end{subfigure}
%     %\hspace{0.2cm}
%     \hfill
%     %
%     \begin{subfigure}[b]{0.55\textwidth}
%     \begin{lstlisting}[breaklines=true, breakatwhitespace=true, basicstyle=\footnotesize\ttfamily, columns=fullflexible]
% int func_270(type_255,type_762)
% {
%     int var_289 = num_463, var_649 = num_199, var_635, var_257, var_165;
%     double var_663, var_792, var_305, var_610, var_55;

%     MPI_Init(&type_255,&type_762);
%     MPI_Comm_size(var_674,&var_257);
%     MPI_Comm_rank(var_674,&var_635);

%     while (!var_289)
%     {
%         MPI_Bcast(&var_649, num_700, var_167, num_463, var_674);
%         if (var_649 == num_463) 
%             break;
%         var_305   = num_302 / (double) var_649;...
%     \end{lstlisting}
%         \caption{Tokompiler source code}
%         \label{fig:subfig2}
%     \end{subfigure}
%     \caption{Pi parallel source code and its corresponding Tokompiler version, which embeds AST information while neglect any semantic information. Tokompiler version is used to demonstrate Monocoder's semantic information independence during generation compared to other models.}
%     \label{fig:tokompiler}
% \end{figure*}
